On the realization of graph as invariant of pseudoharmonic functions

Necessary and sufficient conditions for a finite connected graph with a strict partial order on vertices to be a combinatorial invariant of pseudoharmonic function are obtained.

==> Intro.tex <==
\section*{Вступ}

Класифікація та дослідження умов
топологічної еквівалентності функцій, потоків та інших структур на многовидах є одним з важливих напрямків в топології. Цим питанням присвячені роботи М.
Морса, В. Каплана,  С. Стоілова, В.І. Арнольда, А.Т. Фоменка, В.В.
Шарка, О.В. Болсінова, С.І. Максименка, А.А. Ошемкова, О.О. Пришляка та ін., що охоплюють широкий спектр проблем: класифікацію морсифікацій, гладких функцій з ізольованими особливостями, гамільтонових пото\-ків і т.д. Важливим етапом розв'язання задач такого типу є побудова інваріанту заданої структури, причому у більшості випадків він є деяким комбінаторним об'єктом.

У 40-60-х роках минулого століття з'явилась серія робіт таких класиків, як М.Морс, Дж.Дженкінс, В.Ботсбі та В.Каплан, що присвячені вивченню властивостей гармонічних  та псевдогармонічних функцій. Оскільки, саме ці функції є основним апаратом при розв'язання задач з фізики, механіки та описують багато явищ (потенціал постійного електричного поля в області, що не містить електричних зарядів, потенціал швидкостей безвихрового руху рідини, температура тіла за умов стабілізації розподілу тепла, величина прогину мембрани, що натягнута на контур довільної форми).

Однією з перших була робота Марстона Морса~\cite{Mrt}(1946), що стала основою книги~\cite{Mr}(1951), де автор досліджує поведінку псевдогармонічних функцій, що задані в однозв'язній області, доводить фундаментальну нерівність (нерівність Морса), яка пов'язує числа критичних точок у внутрішності області зі числом локальних екстремумів на межі, а також теореми про локальне представлення околів критичних, межових критичних точок та локальних екстремумів на межі. Зокрема, в роботі~\cite{MrJ} автори  вводять поняття контурної еквівалентності псевдо\-гармонічних функцій, які задані в однозв'язній області. Дві функції є контурно еквівалентні, якщо існує відповідність між лініями рівнів критичних значень. Проте, слід відмітити, що поведінка функції на межі при такій еквівалентності не береться до уваги. Іншими словами, дві контурно еквівалентні функції не є топологічно еквівалентними. Всі подальші роботи були присвячені дослідженню псевдогармо\-нічних функцій на площині, відкритих ріманових поверхнях.

В дисертаційній роботі Андріюк О.П.~\cite{AAnd} було доведено критерій топологічної еквівалентності псевдогармонічних функцій, які задані на диску та приймають \textit{не більш ніж
  одне критичне значення}.

  Дана робота присвячена дослідженню умов топологічної еквівалентності псевдо\-гармонічних функцій, що задані на диску та мають скінченне число локальних екстремумів на межі (дане обмеження є суттєвим, оскільки з нього автоматично слідує скінченність числа критичних точок у внутрішності).

   В першому розділі даної роботи ми будуємо інваріант (комбінаторну діаграму) даних функцій та досліджуємо його властивості. Комбінаторна діаграма -- скінченний, зв'язний граф зі строгим частковим порядком на вершинах. Саме ізоморфізм таких інваріантів є необхідною та достатньою умовою топологічної еквівалентності псевдогармонічних функцій.

   Другий та третій розділи присвячені питанню реалізації деякого комбінаторного об'єкту (скінченного, зв'язного графу зі строгим частковим порядком на вершинах), як діаграми псевдогармонічної функції на диску. Для досягнення цілі, необхідно розв'язати додаткову комбінаторну задачу (якій присвячений другий розділ), яка пов'язана з існуванням вкладення $\phi:T\rightarrow D^{2}$ такого, що $\phi(V^{\ast})\subset \partial D^2$, $\phi(T\setminus V^{\ast})\subset Int D^2$, де $V^{\ast}$ -- підмножина вершин дерева, зі заданим циклічним порядком і містить всі кінцеві вершини. В роботі знайдено критерій існування такого вкладення.

   У третьому розділі сформульовано та доведено теорему про реалізацію. Зрозуміло, що виконання для графа всіх властивостей, зазначених у першому розділі, не достатньо для того, щоб він реалізував діаграму деякої псевдогармонічної функції. Суттєвими є обмеження на строгий частковий порядок на графі, що видно з формулювання теореми 3..

   Висловлюємо щиру подяку Шарку В.В., Максименку С.І та Власенку І.Ю. за корисні поради, обговорення та постійний інтерес до даної задачі.


